Natural Language Processing for Dialects of a Language: A Survey

State-of-the-art natural language processing (NLP) models are trained on massive training corpora, and report a superlative performance on evaluation datasets. This survey delves into an important attribute of these datasets: the dialect of a language. Motivated by the performance degradation of NLP models for dialectal datasets and its implications for the equity of language technologies, we survey past research in NLP for dialects in terms of datasets, and approaches. We describe a wide range of NLP tasks in terms of two categories: natural language understanding (NLU) (for tasks such as dialect classification, sentiment analysis, parsing, and NLU benchmarks) and natural language generation (NLG) (for summarisation, machine translation, and dialogue systems). The survey is also broad in its coverage of languages which include English, Arabic, German, among others. We observe that past work in NLP concerning dialects goes deeper than mere dialect classification, and extends to several NLU and NLG tasks. For these tasks, we describe classical machine learning using statistical models, along with the recent deep learning-based approaches based on pre-trained language models. We expect that this survey will be useful to NLP researchers interested in building equitable language technologies by rethinking LLM benchmarks and model architectures.

==> chaps/7ethical.tex <==
% This file is not used in the final pdf.

\section{Ethical \& Social Considerations}
\label{sec:ethics}
Overall, \redtext{dialectal} NLP presents an excellent avenue for research with huge social implications. We highlight three considerations of relevance.
% This file is not used in the final pdf.
\subsection{Social Implications}
\redtext{People who speak the same dialect may feel a strong social connection.} Furthermore, certain traditions and practices are tied to localities which are in turn tied to dialects. If the goal of NLP research is to make communication seamless then the only correct way to do so is via a strong emphasis on dialects. There is also a growing concern among speakers of specific dialects that their language is dying due to the pervasiveness of English via the internet. As NLP researchers, we should acknowledge these concerns and make headway into preserving as many dialects as possible, at the risk of losing valuable aspects of the vast tapestry of culture and history.

\subsection{\redtext{dialectal} Research By Dialect Speakers}
Linguistic research colonization is the process where researchers who do not speak specific languages nor have connections with them conduct research on said languages. Despite the negative connotation of colonization, this is not a bad thing, because no one should monopolize working on specific languages. However, it highlights that there are haves and have-nots, where the haves are researchers and organizations with funding who can work on dialects and the have-nots are the researchers who would like to work on dialects but simply lack funding. Recently, there has been a growing trend where language speakers are reclaiming dominion over research involving their own languages. For example, there has been an explosive growth in the number of researchers and groups like DeepLearning Indaba, Masakhane from African countries working solely on African languages and organizations like AI4Bharat in India working on Indian languages. Indeed, they have shown that dedicated focus on language research by speakers of these languages lead to better NLP systems. We therefore propose that the organizations with funding leverage their privilege and support those without funding so as to ensure that work on dialects is led and owned by groups that are most connected and impacted by dialects. This will lead to true diversity and inclusivity in NLP research which will strongly impact society.

\subsection{Normalizing Working on and Speaking Dialects}
One aspect which limits \redtext{dialectal} research is the concept of shame in speaking a certain language or a dialect, an aspect which is also known as linguistic self-hatred\footnote{\url{https://unravellingmag.com/articles/linguistic-self-hate/}; Accessed on 9th January, 2024.}\footnote{\url{https://languagehat.com/linguistic-self-hatred/}; Accessed on 9th January, 2024.}. For example, take the case of Mauritian creole, whose speakers are dwindling by the day, mainly because the younger generation feels shame\footnote{\url{https://lexpress.mu/blog/286734/creole-disillusion}; Accessed on 11th December 2023.} in speaking their native language. The same exists for Konkani\footnote{\url{https://hanvkonn.wordpress.com/2019/06/22/ashamed-of-speaking-in-konkani/}; Accessed on 11th December 2023}. While there are no official reports highlighting the same for dialects, it is not farfetched to consider that linguistic self-hatred will exist here as well. It is time to end this self-hatred and normalize speaking dialects. By doing so, people speaking dialects will become more enthusiastic about preserving their dialects and this will inevitably aid research on dialects, thereby positively impacting society. Dialects are closely tied to culture and such differences have not been captured explicitly beyond the works described in this paper.% This file is not used in the final pdf.

==> tables/table-dialclassapproaches.tex <==
\begin{table}[]
\begin{tabular}{lll}\toprule
\textbf{Paper} & \textbf{Language}         & \textbf{Approach}        \\ \midrule
~\cite{chitturi-hansen-2008-dialect} & English & Acoustic features\\
~\cite{lui2013classifying} & English & n-grams \& POS n-grams \\
~\cite{darwish-etal-2014-verifiably} & Arabic & Phonological, lexical, morphological \\ 
~\cite{dogruoz-nakov-2014-predicting} & Turkish & Verbs and associated markers \\
~\cite{simaki-etal-2017-identifying} & English & Lexical, Morphological, ... \\
~\cite{criscuolo2017discriminating} & Multiple & Character embeddings \\
~\cite{jurgens-etal-2017-incorporating} & Multiple & Seq-to-seq modeling of character embeddings \\
~\cite{abdul2018you} & Arabic & Localised word embeddings \\
\redtext{~\cite{salameh2018fine}} & Arabic & \redtext{Word and character n-grams} \\
~\cite{goswami2020unsupervised} & German & Unsupervised character-to-sentence embeddings\\
~\cite{ramponi2023diatopit} & Italian & Fine-tuned LLMs\\
~\cite{obeid2020camel} & Arabic & Fine-tuned LLMs\\
\bottomrule   
\end{tabular}
\caption{Dialect Classification Approaches; `Languages' refers to the language whose dialects are considered.}
\label{tab:dialectclassification}
\end{table}

==> tables/table-langdist-removed.tex <==
\begin{table}[]
\begin{tabular}{ll}
\toprule
\textbf{Paper}                       & \textbf{Source languages}                               \\ \midrule
~\cite{farha2022effect} & Dialects of Arabic \\
~\cite{lui2013classifying} & Dialects of English \\
~\cite{simaki-etal-2017-identifying} & Dialects of English \\
~\cite{hanani2020spoken} & Dialect of Arabic \\
~\cite{goswami2020unsupervised} & Dialect of German \\
~\cite{hou2020classification} & Dialects of Chinese \\
~\cite{abdul2018you} & Dialects of Arabic \\
~\cite{blodgett-etal-2016-demographic} & Dialect of English \\
~\cite{barnes-etal-2021-nordial} & Dialects of Norwegian \\
~\cite{aji-etal-2022-one} & Dialects of Indonesian \\
~\cite{ramponi2023diatopit} & Dialects of Italian \\ \bottomrule
\end{tabular}
\caption{Language distribution for dialect detection.}
\label{tab:dialectid1}
\end{table}

==> tables/table-needtofind_no.tex <==
\begin{table*}[]
\begin{tabular}{lcccc}
\toprule
\textbf{Paper} & \multicolumn{3}{c}{Language/Dialects} & Approach \\ \midrule
     & Chinese & Arabic      & German      &     \\ \midrule
~\cite{hou2020classification}  & \OK     &    -    &  - & - \\ 
~\cite{kanjirangat2022early} & & \OK & \OK & \OK \\
 \bottomrule
\end{tabular}
\caption{Need to find out}
\end{table*}
